Matrix Approximation with Side Information: When Column Sampling is Enough

A novel matrix approximation problem is considered herein: observations based on a few fully sampled columns and quasi-polynomial structural side information are exploited. The framework is motivated by quantum chemistry problems wherein full matrix computation is expensive, and partial computations only lead to column information. The proposed algorithm successfully estimates the column and row-space of a true matrix given a priori structural knowledge of the true matrix. A theoretical spectral error bound is provided, which captures the possible inaccuracies of the side information. The error bound proves it scales in its signal-to-noise (SNR) ratio. The proposed algorithm is validated via simulations which enable the characterization of the amount of information provided by the quasi-polynomial side information.

==> intro_old.tex <==

In the various applications of computer vision, machine learning and chemical physics, a matrix is common way to represent the data. Examples include such as scientific computing \cite{quiton_pvmc_2022,quiton_matrix_2020}, sensor localization \cite{}, recommendation systems\cite{}. It is a common scenario that some of entries in a matrix are not collected and missing\cite{}.

To address this problem, many of matrix completion algorithms have been proposed for decades \cite{}. Conventional matrix completion has been extensively studied under the uniform sampling assumption where the missing entries are distributed uniformly at random \cite{}. Recently, however, many applications of computer vision, bioinformatics and data science \cite{cai2016structured,foucart2020weighted,gunasekar2015unified,hu2018generalized} show that the sampling pattern may not be obtained uniformly at random. In this case, random- sampling based matrix completion can not be directly applied. Therefore, new reconstruction strategies are required. 


This work addresses a column sampled matrix reconstruction problem coupled with side information on the row-space of the true matrix versus the typical random sampling. Figure~\ref{fig:sampling} illustrates the example of column-based sampling.  The sampling strategy is motivated by quantum chemistry \cite{quiton_pvmc_2022,quiton_matrix_2020,bac2022matrix}, where full matrix computation is expensive and only full columns can be
computed. As shown in \cite{candes2009}, one could never guess the value of components, by any method if no information for them is given. To  recover an unknown matrix, one needs at least one observation per row and one observation per column. For non-uniform sampling matrix recovery problems,
\cite{foucart2020weighted} proposes a weighted matrix based method, which solves for the estimated matrix %that minimize
%\begin{align}
%    \min\Vert {\bf H} \circ ({\bf M} - \hat{\bf M})\Vert_{F}^{2}.
%\end{align} 
given a fixed non-uniform sampling pattern and weight matrix.
\begin{figure}[!h]
    \centering
\includegraphics[width=8cm]{sampling.png}
    \caption{An example of random sampling and column-based sampling when a matrix ${\bf M} \in \RR^{5 \times 9}$. The black entries indicate observed samples.}
   \label{fig:sampling}
\end{figure}


\cite{liu2017new} studied a nonuniform sampling matrix completion and introduces isomeric condition, which relates the rank and coherence with the locations and amount of the observed entries. However, the setup of \cite{liu2017new} still considers few entries sampled in each column and the algorithm is built on non-convex setting, which are different from our set up. For non-uniform sampling problems, one can think of performing a matrix completion algorithm with columns but most matrix completion algorithms consider randomly selected entries and also it assumes a target matrix is low rank, which works poorly in our full-rank assumption.  

%\cite{drineas2008relative,mahoney2009cur} propose CUR decomposition methods which perform low-rank matrix decomposition using the subspace information constructed by the actual columns and rows of the target matrix. 


% However, all the existing CUR algorithms require the knowledge of every entry in the target matrix \cite{} and they cannot deal with a case where only columns or rows are sampled, while it is found in real application. 
CUR+ algorithm \cite{xu2015cur} allows for the sampling of complete columns and rows as well as some additional random samples. Although it is the most similar work to our problem among the literature, there is a big difference that it also necessitates fully sampled rows as well as additional random samples to estimate its row space, thus, \cite{xu2015cur} cannot be applied to our quantum chemistry problem either. To the best of our knowledge, matrix approximation with column samples and rowspace information as captured by a quasi-polynomial structure has not been previously investigated. 

The proposed algorithm, dubbed quasi- polynomial matrix approximation (QPMA), computes the low rank approximation of the target matrix based on (i) the randomly sampled columns (or rows) and (ii) a known quasi-polynomial side information of a true matrix.\\ 
\noindent{\bf Contribution}
A new framework for matrix approximation given only a few columns and quasi-polynomial side information is proposed. A theoretical additive error bound is provided and shown to be comparable to that achieved by conventional matrix approximation methods. Simulation studies validate that the estimated rowspace information provided by QPMA provides useful side information and enables the characterization of how much information is provided via the quasi-polynomial structure.

==> related.tex <==

\vspace{0.2cm}
{{\section{Related methods}}}
\label{sec:prior}



This paper is closely related to series of papers in matrix completion and approximation.






In matrix approximation problems, the goal is to construct a low rank-$r$ version matrix $\hat{\mathbf{M}}$ of a true matrix $\mathbf{M}$ with a true rank $k$ where $r \leq k$. To do this, a subset of columns or low rank column and row space information is given \cite{xu2015cur}.  \jm{Add more citations} The additive error guarantee is commonly used for performance measure defined as
\begin{align}\label{eq:additive_error}
    \left\Vert \mathbf{M}-\hat{\mathbf{M}}\right\Vert_{F} \leq \left\Vert \mathbf{M}-\mathbf{M}_{r}\right\Vert_{F} +\epsilon\left\Vert \mathbf{M}\right\Vert_{F},
\end{align} where $\mathbf{M}_{r}$ is the best rank-$r$ approximation of a matrix $\mathbf{M}$ and $0\leq\epsilon\leq1$.
Ideally, we want to construct $\hat{\mathbf{M}}$, that is close to $\mathbf{M}_{r}$. Recently, \cite{xu2015cur} proposed an algorithm called CUR+, which samples $d$ full columns and $d$ rows and some randomly sampled entries of a matrix $\mathbf{M} \in \RR^{n \times m}$ and showed the error bound with the sample complexity $O(nr\ln r)$.   
%Given a target rank $r$, the $d$ number of sampled columns and rows and $O(r^2\ln r)$ randomly sampled entries, the error bound of CUR+ is given by 
%\begin{align}
%    \left\Vert \mathbf{M}-\hat{\mathbf{M}} \right\Vert_2^2 \leq 8\sigma^2_{r+1}(\mathbf{M})(1+2mn)\left(1+\frac{n+m}{d}\right),\nonumber
%\end{align} where $\sigma^2_{r+1}(\mathbf{M})$ indicates the $r+1$ largest singular value of $\mathbf{M}$.
Despite the great theoretical guarantees and performances of prior works, the limitation is either the true matrix or true column and row space is provided, which can not be directly applied into our problem. A low rank matrix approximation problem with a few columns  without knowing full true matrix has not been considered in none of these work.

To this end, this paper studies a column-sampled matrix problem for the first time in the matrix completion and approximation literature. We provide a column sampling complexity and spectral error bound between the true matrix and a reconstructed matrix. Our proposed method assumes noisy side information on the structure of the true matrix and investigates the performance based on the noisiness of the true matrix. 


==> related_old.tex <==

\vspace{0.2cm}
{{\section{Related methods}}}
\label{sec:prior}

{\pn{on a high level, the related methods section has two main parts - matrix completion and matrix approximation. \\
for MC, we briefly mention that most works consider the uniform at random sampling model, and provide a brief description of best known results for convex relaxation, and non-convex approaches. mention the pros and cons for each of them. \\
Next, there is also a plethora of MC papers that considers non-uniform sampling (there are also papers that consider column sampling type resuls (some of them are called outlier robust mc/pca). we need to do a thorough literature search for this and try to distill the information from these papers. another slightly related works is based on side-information for the MC problem itself, this also needs to be thorough, since this is closest to our work. \\
finally, we discuss the matrix approximation literature. this can be anything from sketching, to matrix sensing style results, to other problem formulations that you have kind of mentioned here. For all of these, we briefly mention the flavor of results obtained. I do not think here we need to discuss elaborately on convex relaxation vs non-convex approaches, (since the convex relaxations are all a special case of min rank matrix linear equations discussed in recht and fazel) but we can certainly mention them briefly. \\
all the above should lead to the type of additive error results that we finally obtain, and should do a good job of placing the paper in good context. }}

This paper is closely related to series of papers in matrix completion and approximation.

Most of standard matrix completion work assume that the observed entries are uniformly sampled at random \cite{candes_exact_2009,candes2010matrix}. These works provide the theoretical guarantees that $O(nr\mu \poly\log n)$ observations are sufficient for exact recovery for a $n \times n$ matrix of rank $r$ under the assumptions that the coherences of row and column subspace are bounded by some small positive value. These results involve the coherence $\mu$, implying that both column and row space of a true matrix must be coherent. In our problem, however, rowspace information is very limited, thus we do not have an access to true coherence value. In Theorem~\ref{eq:thm1}, we show that the matrix can be recovered when a given side information matrix provides a rowspace information that is close to a true matrix. 

Several studies consider a matrix completion with side information such as its graph structure or feature information of data to help complete the matrix \cite{elmahdy2020matrix,chiang2015matrix,xu2013speedup,zhang2019inductive,menon2011response,natarajan2014inductive}. In the Netflix problem, for example,  profiles of users or genre of movies might also be given, and one could possibly leverage such side information for better prediction. \cite{xu2013speedup,natarajan2014inductive,chiang2015matrix} show that recovery could be attained with lower sample complexity when row space and column space information is given. However, there are two main limitations of these works. One is that all of them consider the case when observed entries are randomly sampled and the other is that the side information on row and column space is assumed to be perfect. While \cite{chiang2015matrix} studied when imperfect side information is given, but still the observations are uniformly sampled at random.

Recently, due to the growing amount of necessity of nonuniformly sampled matrix completion problem, especially in economics \cite{farias2021learning}, magnetic resonance imaging \cite{liu2017new} and quantum chemistry \cite{quiton_pvmc_2022}, there is sparse literature studying nonuniform sampling matrix completion problem \cite{foucart2020weighted,negahban2012restricted,liu2017new,xu2015cur}. For example, \cite{liu2017new} investigated a situation where locations of the observed entries are concentrated around the main diagonal of a matrix and suggested a new hypothesis called isomeric condition that guarantees a recovery of the matrix sampled irregularly. However, none of these work considers column-sampled matrix completion problem. 

In matrix approximation problems, the goal is to construct a low rank-$r$ version matrix $\hat{\mathbf{M}}$ of a true matrix $\mathbf{M}$ with a true rank $k$ where $r \leq k$. To do this, a subset of columns or low rank column and row space information is given \cite{xu2015cur}.  \jm{Add more citations} The additive error guarantee is commonly used for performance measure defined as
\begin{align}\label{eq:additive_error}
    \left\Vert \mathbf{M}-\hat{\mathbf{M}}\right\Vert_{F} \leq \left\Vert \mathbf{M}-\mathbf{M}_{r}\right\Vert_{F} +\epsilon\left\Vert \mathbf{M}\right\Vert_{F},
\end{align} where $\mathbf{M}_{r}$ is the best rank-$r$ approximation of a matrix $\mathbf{M}$ and $0\leq\epsilon\leq1$.
Ideally, we want to construct $\hat{\mathbf{M}}$, that is close to $\mathbf{M}_{r}$. Recently, \cite{xu2015cur} proposed an algorithm called CUR+, which samples $d$ full columns and $d$ rows and some randomly sampled entries of a matrix $\mathbf{M} \in \RR^{n \times m}$ and showed the error bound with the sample complexity $O(nr\ln r)$.   
%Given a target rank $r$, the $d$ number of sampled columns and rows and $O(r^2\ln r)$ randomly sampled entries, the error bound of CUR+ is given by 
%\begin{align}
%    \left\Vert \mathbf{M}-\hat{\mathbf{M}} \right\Vert_2^2 \leq 8\sigma^2_{r+1}(\mathbf{M})(1+2mn)\left(1+\frac{n+m}{d}\right),\nonumber
%\end{align} where $\sigma^2_{r+1}(\mathbf{M})$ indicates the $r+1$ largest singular value of $\mathbf{M}$.
Despite the great theoretical guarantees and performances of prior works, the limitation is either the true matrix or true column and row space is provided, which can not be directly applied into our problem. A low rank matrix approximation problem with a few columns  without knowing full true matrix has not been considered in none of these work.

To this end, this paper studies a column-sampled matrix problem for the first time in the matrix completion and approximation literature. We provide a column sampling complexity and spectral error bound between the true matrix and a reconstructed matrix. Our proposed method assumes noisy side information on the structure of the true matrix and investigates the performance based on the noisiness of the true matrix. 

%\subsection{Randomly sampled matrix completion} The original work \cite{} on matrix completion sought to estimate the missing entries of a low rank matrix based on uniformly, randomly observed entries. The needed sampling complexity of this early work was $O(n^{1.2}r \ln n)$, where $r$ is the rank of the true matrix with dimension  $n \times n$. The proposed strategy was based on minimizing the nuclear norm 
%\cite{candes_exact_2009,candes_exact_2012},
%\begin{align}
%    \min {\Vert {\bf X}\Vert}_{*} \;\; \mbox{subject to} \; {\bf X}_{ij} = {\bf M}_{ij}, (i,j) \in \Omega \nonumber,
%\end{align} {where $\Omega \subset [n] \times [m]$ is the index set of observed entries} and ${\Vert {\bf X}\Vert}_{*}$, the nuclear norm, is the sum of the singular values of {\bf X}.

%{{Let the singular value decomposition of the true matrix {\bf M} be ${\bf U}{\bf \Sigma} {\bf V}^{\trasp}$, where  ${\bf U} \in \RR^{n \times r}, {\bf \Sigma} \in \RR^{r \times r} \; \mbox{and}\; {\bf V} \in \RR^{m \times r}$ respectively.}}
%An important measure of the hardness of matrix completion is the coherence measure, defined as 
%{{
%\begin{align}
%    \mu({\bf U}) \equiv \frac{n}{r}\max_{1\leq i \leq n} {\Vert {\bf P}_U {\bf e}_{i} \Vert}^2\nonumber,
%\end{align}
%where ${\bf P}_U$ is an orthogonal projection onto {\bf U} and ${\bf e}_{i}$ is a standard basis vector. It is desired that the singular vectors have sufficient spread with respect to the standard basis vectors, so that each singular vector is equally informative about the matrix {\bf M}  \cite{candes_exact_2009}.  This level of relative spread is captured by the coherence, and a low coherence is desired. Not surprisingly, the number of samples needed (sample complexity) for accurate recovery is governed by the coherence. With appropriately low coherence of the row and column subspaces, a matrix can be recovered with high probability.   We will characterize the impact of the side information matrix on coherence and thus sample complexity for our problem statement. }}

 


%\subsection{Column and row sampled matrix approximation} %In contrast to matrix {\bf completion}, there is recent work on matrix {\bf approximation} using complete column and row information, where these vectors are randomly sampled from the original matrix \cite{drineas2008relative,mahoney2009cur,boutsidis2017optimal,boutsidis2014near,xu2015cur}. The main goal of these works is to compute low rank approximations, that is, the original matrix itself may not be low rank. For example, \cite{mahoney2009cur} randomly samples $d_1$ columns and $d_2$ rows from an input matrix {\bf M} and constructs matrices {\bf C} and {\bf R } from these sampled columns and rows. Given an input matrix {\bf M}, {\bf C}, {\bf R} and a rank parameter $r$, the CUR algorithm \cite{mahoney2009cur} approximates its low-rank matrix as $\hat{{\bf M}}$ = ${\bf C\bf U\bf R}$, where {\bf U} is a carefully designed matrix that guarantees that its approximation is close to {\bf M}. However, full information of a target matrix {\bf M} is required to obtain {\bf U}, which we cannot directly apply this strategy to our chemical rate reaction problem.

%Recently, the CUR+ method \cite{xu2015cur} is proposed which reconstructs a low rank matrix using $d_1$ randomly sampled columns and $d_2$ randomly sampled rows and some randomly sampled entries. There is an additional operator to randomly sample components from the unsampled columns and rows; the matrix $\Omega$ captures the index set of randomized sampled entries from the unsampled columns and rows. Thus, CUR+ requires at least a total of $d_1m + d_2n-d_1d_2 + |\Omega|$ sample.  If we assume that $d_1=d_2$, the CUR+ method solves 
%\begin{align}
%    \min_{\bf Z} \Vert \mathcal{P}_{\Omega}({\bf M})-\mathcal{P}_{\Omega}(\hat{\bf U}{\bf Z}\hat{\bf V}^{\trasp})\Vert_F^2\nonumber,
%\end{align} where $\hat{\bf U}$ and $\hat{\bf V}$ represent the approximated column and row space of $\mathbf{M}$ and $\mathbf{P}_{\Omega}$ is a projection operator \begin{align}
%    \mathcal{P}_{\Omega}(\mathbf{M})=
%    \begin{cases}
%     {M}_{i,j}\; \mbox{if}\; (i,j) \in \Omega \\
%     0, \; \mbox{otherwise}.
%    \end{cases}
%\end{align}
%Given a target rank $r$, the number of sampled columns and rows $d_1=d_2=d$, $d \geq O(r \ln r)$, and the randomly sampled entries $\Omega$, $|\Omega| \geq O(r^2 \ln r)$, the error bound of CUR+ \cite{xu2015cur} is given by  
%\begin{align}\label{eq:cur_error}
%    {\Vert\mathbf{M}-{\bf \hat{M}_{cur}}\Vert}_{2}^{2} &\leq 8\sigma_{r+1}^2({\bf M})\left(1+2mn\right)\left(1+\frac{n+m}{d}\right)\nonumber,
%\end{align} where $\sigma_{r+1}^{2}$ indicates the $r+1$ largest singular value of $\mathbf{M}$. The sampling complexity of CUR+ is therefore $O(nr\ln r)$ because $O(nr\ln r) \geq nd+\vert \Omega \vert=O(nr\ln r)+ O(r^2 \ln r)$.  Similarly to CUR,  we cannot directly apply CUR+ to our problem as we only have access to columns sampled from $\mathbf{M}$. {However, these schemes will provide good baseline comparisons and enable understanding the amount of information afforded by our side information matrix.}

\vspace{0.2cm}
